An ASP semantics for Constraints involving Conditional Aggregates

We elaborate upon the formal foundations of hybrid Answer Set Programming (ASP) and extend its underlying logical framework with aggregate functions over constraint values and variables. This is achieved by introducing the construct of conditional expressions, which allow for considering two alternatives while evaluating constraints. Which alternative is considered is interpretation-dependent and chosen according to an associated condition. We put some emphasis on logic programs with linear constraints and show how common ASP aggregates can be regarded as particular cases of so-called conditional linear constraints. Finally, we introduce a polynomial-size, modular and faithful translation from our framework into regular (condition-free) Constraint ASP, outlining an implementation of conditional aggregates on top of existing hybrid ASP solvers.

==> proofs/proof_cor_htcc_eqstab.tex <==
\begin{itemize}
  \item \textbf{Proof of Corollary~\ref{cor:htcc:eqstab}}
      \begin{itemize}
          \item Corollary~\ref{cor:htcc:eqstab} follows directly from Proposition~\ref{prop:htcc:reduct}
          \item If $\langle t,t \rangle$ is an equilibrium model of $\varphi$, we know that $\langle t,t \rangle\modelsf\varphi$ and, by Proposition~\ref{prop:htcc:reduct},
                $t\modelscl\varphi^t$
          \item Furthermore, there cannot exist an valuation $h\subset t$ so that $h\modelscl \varphi^t$ since that would imply $\langle h,t \rangle \modelsf \varphi$ again by Proposition~\ref{prop:htcc:reduct},
                 which cannot hold since interpretation $\langle t,t \rangle$ is an equilibrium model of formula $\varphi$ 
          \item Thus, valuation $t$ is a subset minimal model of $\varphi^t$ making it a stable model of $\varphi$ 
          \item Similarly, if valuation $t$ is a stable model of $\varphi$, we know that $t\modelscl \varphi^t$ and $\langle t,t \rangle\modelsf\varphi$ by Proposition~\ref{prop:htcc:reduct} 
          \item Again, there cannot exist an $h\subset t$ such that $\langle h,t \rangle\modelsf\varphi$, because it implies $h\modelscl\varphi^t$ by Proposition~\ref{prop:htcc:reduct},
                which cannot hold since $t$ is a stable model of $\varphi$
          \item In conclusion, $\langle t,t \rangle \modelsf \varphi$ and there exists no $h\subset t$ such that $\langle h,t \rangle\models\varphi$,
                therefore, $\langle t,t \rangle$ is an equilibrium model of $\varphi$
      \end{itemize}       
\end{itemize}

==> proofs/proof_htcc_satisfaction.old.tex <==
\paragraph{Proof of Proposition~\ref{prop:htcc:satisfaction.old}}

\begin{itemize}
\item In the following proof sketch for Proposition~\ref{prop:htcc:satisfaction.old}, we focus on Condition 2.
  The full proof is obtained via structural induction with the remaining conditions that are not subject to change and therefore trivially fulfilled.
\item (Induction base Proposition~\ref{prop:htcc:satisfaction.old}) For $\varphi=c$, we get
  \begin{align}
    &\langle h,t \rangle \models c\label{eq:prop:42}\\
    \text{iff }& h\in \den{c} \text{ and } t\in \den{c}\label{eq:prop:43}\\
    \text{iff }& h\in \den{c}\label{eq:prop:44}\\
    \text{iff }&t\models' c\label{eq:prop:45}
  \end{align}
  \begin{itemize}
  \item Equivalence between \eqref{eq:prop:42} and \eqref{eq:prop:43} holds by definition of the satisfaction relation $\models$
  \item Equivalence between \eqref{eq:prop:43} and \eqref{eq:prop:44} holds since the denotation of $c$ is closed and therefore $h\in\den{c}$ implies $t\in\den{c}$ for all valuations $h\subseteq t$
  \item Equivalence between \eqref{eq:prop:44} and \eqref{eq:prop:45} holds by definition of the classical satisfaction relation $\models'$
  \end{itemize}
\end{itemize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> proofs/proof_lem_htcc_confree.tex <==
\begin{itemize}
  \item \textbf{Proof of Lemma~\ref{lem:htcc:confree}}
    \begin{itemize}
     \item We proof Lemma~\ref{lem:htcc:confree} via induction over the structure of the formula
     \item (Induction base) For condition-free constraint atom $c$, we get
      \begin{align}
                & \langle h,t\rangle\modelsf c \label{eq:lem:61} \\
\text{iff } & h\in\den{\evalf{h}{t}(c)}\text{ and }t\in\den{\evalf{t}{t}(c)}\label{eq:confreeht} \\
\text{iff } & h\in\den{\evalcl{h}(c)}\text{ and }t\in\den{\evalcl{t}(c)}\label{eq:confreefer} \\
\text{iff } & h\modelscl c\text{ and }t\modelscl c \label{eq:lem:62} \\
\text{iff } & h\modelscl c^t  \label{eq:lem:63} 
      \end{align} 
          \begin{itemize}
           \item 
          Equivalence between \eqref{eq:lem:61} and \eqref{eq:confreeht} holds by definition of the satisfaction relation
           \item 
          Equivalence between \eqref{eq:confreeht} and \eqref{eq:confreefer} holds by definition of the evaluation function 
          since $\evalf{v}{v'}(c)=\evalcl{v''}(c)=c$ for any condition-free constraint $c$ and valuations $v,v',v''$
           \item 
          Equivalence between \eqref{eq:confreefer} and \eqref{eq:lem:62} holds by definition of the classical satisfaction relation
           \item 
          Equivalence between \eqref{eq:lem:62} and \eqref{eq:lem:63} holds by definition of the reduct 
          since $c^t=c$ for any condition-free constraint atom $c$ such that $t\modelscl c$,
          which in turn has to hold since otherwise $h$ is no classical model of $c^t$
          \end{itemize}     
          \item (Induction step) For formula $\varphi_1 \land \varphi_2$, we get
          \begin{align}
               &\langle h,t \rangle \modelsf \varphi_1 \land \varphi_2\label{eq:lem:71}\\
\text{iff }&\langle h,t \rangle \modelsf \varphi_1\text{ and }\langle h,t \rangle \modelsf \varphi_2\label{eq:lem:72}\\
\text{iff }&h\modelscl \varphi_1^t\text{ and }h \modelscl \varphi_2^t\label{eq:lem:73}\\
\text{iff }&h\modelscl (\varphi_1\land \varphi_2)^t\label{eq:lem:74}
          \end{align}
          \begin{itemize}
           \item Equivalence between \eqref{eq:lem:71} and \eqref{eq:lem:72} holds by definition of the satisfaction relation
           \item Equivalence between \eqref{eq:lem:72} and \eqref{eq:lem:73} holds by induction hypothesis
           \item Equivalence between \eqref{eq:lem:73} and \eqref{eq:lem:74} holds by definitions of the classical satisfaction relation and reduct
          \end{itemize}
          \item (Induction step) For formula $\varphi_1 \lor \varphi_2$, we get
          \begin{align}
               &\langle h,t \rangle \modelsf \varphi_1 \lor \varphi_2\label{eq:lem:81}\\
\text{iff }&\langle h,t \rangle \modelsf \varphi_1\text{ or }\langle h,t \rangle \modelsf \varphi_2\label{eq:lem:82}\\
\text{iff }&h\modelscl \varphi_1^t\text{ or }h \modelscl \varphi_2^t\label{eq:lem:83}\\
\text{iff }&h\modelscl (\varphi_1\lor \varphi_2)^t\label{eq:lem:84}
          \end{align}
          \begin{itemize}
           \item Equivalence between \eqref{eq:lem:81} and \eqref{eq:lem:82} holds by definition of the satisfaction relation
           \item Equivalence between \eqref{eq:lem:82} and \eqref{eq:lem:83} holds by induction hypothesis
           \item Equivalence between \eqref{eq:lem:83} and \eqref{eq:lem:84} holds by definitions of the classical satisfaction relation and reduct
          \end{itemize}
          \item (Induction step) For formula $\varphi_1 \rightarrow \varphi_2$, we get
          \begin{align}
               &\langle h,t \rangle \modelsf \varphi_1 \rightarrow \varphi_2\label{eq:lem:91}\\
\text{iff }&\langle h,t \rangle \not\modelsf \varphi_1\text{ or }\langle h,t \rangle \modelsf \varphi_2\text{, and }\langle t,t \rangle \models \varphi_1 \rightarrow \varphi_2\label{eq:lem:92}\\
\text{iff }&h \not\modelscl \varphi_1^t\text{ or }h \modelscl \varphi_2^t\text{, and }t \modelscl \varphi_1 \rightarrow \varphi_2\label{eq:lem:93}\\
\text{iff }&h\modelscl (\varphi_1 \rightarrow \varphi_2)^t\label{eq:lem:94}
          \end{align}
          \begin{itemize}
           \item Equivalence between \eqref{eq:lem:91} and \eqref{eq:lem:92} holds by definition of the satisfaction relation and Proposition~\ref{prop:htcc:persistence}
           \item Equivalence between \eqref{eq:lem:92} and \eqref{eq:lem:93} holds by induction hypothesis and Lemma~\ref{lem:htcc:modelscl}
           \item Equivalence between \eqref{eq:lem:93} and \eqref{eq:lem:94} holds by definitions of the classical satisfaction relation and reduct
          \end{itemize}
    \end{itemize}
\end{itemize}

==> proofs/proof_lem_htcc_evalcl+modelscl.tex <==
\begin{itemize}
  \item \textbf{Proof of Lemma~\ref{lem:htcc:evalcl} and Lemma~\ref{lem:htcc:modelscl}}
      \begin{itemize}
          \item We proof Lemma~\ref{lem:htcc:evalcl} and Lemma~\ref{lem:htcc:modelscl} simultaneously via induction over the structure of the formula
          \item (Induction base Lemma~\ref{lem:htcc:evalcl}) For condition-free constraint atom $c$, Lemma~\ref{lem:htcc:evalcl} obviously holds since by definition $\evalf{t}{t}(c)=c$ and $\evalcl{t}(c)=c$
          \item (Induction base Lemma~\ref{lem:htcc:modelscl}) For condition-free constraint atom $c$, we get
          \begin{align}
               &\langle t,t \rangle \modelsf c\label{eq:lem:1}\\
\text{iff }&t\in\den{\evalf{t}{t}(c)}\label{eq:lem:evaleq}\\
\text{iff }&t\in\den{\evalcl{t}(c)}\label{eq:lem:evalcleq}\\
\text{iff }&t\modelscl c\label{eq:lem:4}
          \end{align}
          \begin{itemize}
           \item Equivalence between \eqref{eq:lem:1} and \eqref{eq:lem:evaleq} holds by definition of the satisfaction relation
           \item Equivalence between \eqref{eq:lem:evaleq} and \eqref{eq:lem:evalcleq} holds since $\evalf{t}{t}(c)=\evalcl{t}(c)$ for any interpretation $\langle t,t \rangle$ and condition-free $c$ as shown above
           \item Equivalence between \eqref{eq:lem:evalcleq} and \eqref{eq:lem:4} holds by definition of the classical satisfaction relation
          \end{itemize}

                    
          \item (Induction step Lemma~\ref{lem:htcc:evalcl}) For conditional constraint atom $c$, we have
          \begin{align*}
          &\evalf{t}{t}(c[\cterm{r_1}{s_1}{\varphi_1},\dots,\cterm{r_n}{s_n}{\varphi_n}])=\\
          &\quad c[\evalf{t}{t}(\cterm{r_1}{s_1}{\varphi_1}),\dots,\evalf{t}{t}(\cterm{r_n}{s_n}{\varphi_n})]
          \end{align*}
          and
          \begin{align*}
          &\evalcl{t}(c[\cterm{r_1}{s_1}{\varphi_1},\dots,\cterm{r_n}{s_n}{\varphi_n}])=\\
          &\quad c[\evalcl{t}(\cterm{r_1}{s_1}{\varphi_1}),\dots,\evalcl{t}(\cterm{r_n}{s_n}{\varphi_n})],
          \end{align*}
          thus, $\evalf{t}{t}(c)=\evalcl{t}(c)$ in case that $\langle t,t \rangle\modelsf\varphi_i$ iff $t\modelscl\varphi_i$ for $1\leq i\leq n$,
          which holds by induction hypothesis
          \item (Induction step Lemma~\ref{lem:htcc:modelscl}) For formula $\varphi_1 \land \varphi_2$, we get
          \begin{align}
               &\langle t,t \rangle \modelsf \varphi_1 \land \varphi_2\label{eq:lem:21}\\
\text{iff }&\langle t,t \rangle \modelsf \varphi_1\text{ and }\langle t,t \rangle \modelsf \varphi_2\label{eq:lem:22}\\
\text{iff }&t\modelscl \varphi_1\text{ and }t \modelscl \varphi_2\label{eq:lem:23}\\
\text{iff }&t\modelscl \varphi_1\land \varphi_2\label{eq:lem:24}
          \end{align}
          \begin{itemize}
           \item Equivalence between \eqref{eq:lem:21} and \eqref{eq:lem:22} holds by definition of the satisfaction relation
           \item Equivalence between \eqref{eq:lem:22} and \eqref{eq:lem:23} holds by induction hypothesis
           \item Equivalence between \eqref{eq:lem:23} and \eqref{eq:lem:24} holds by definition of the classical satisfaction relation
          \end{itemize}
          \item (Induction step Lemma~\ref{lem:htcc:modelscl}) For formula $\varphi_1 \lor \varphi_2$, we get
          \begin{align}
               &\langle t,t \rangle \modelsf \varphi_1 \lor \varphi_2\label{eq:lem:31}\\
\text{iff }&\langle t,t \rangle \modelsf \varphi_1\text{ or }\langle t,t \rangle \modelsf \varphi_2\label{eq:lem:32}\\
\text{iff }&t\modelscl \varphi_1\text{ or }t \modelscl \varphi_2\label{eq:lem:33}\\
\text{iff }&t\modelscl \varphi_1\lor \varphi_2\label{eq:lem:34}
          \end{align}
          \begin{itemize}
           \item Equivalence between \eqref{eq:lem:31} and \eqref{eq:lem:32} holds by definition of the satisfaction relation
           \item Equivalence between \eqref{eq:lem:32} and \eqref{eq:lem:33} holds by induction hypothesis
           \item Equivalence between \eqref{eq:lem:33} and \eqref{eq:lem:34} holds by definition of the classical satisfaction relation
          \end{itemize}
          \item (Induction step Lemma~\ref{lem:htcc:modelscl}) For formula $\varphi_1 \rightarrow \varphi_2$, we get
          \begin{align}
               &\langle t,t \rangle \modelsf \varphi_1 \rightarrow \varphi_2\label{eq:lem:41}\\
\text{iff }&\langle t,t \rangle \not\modelsf \varphi_1\text{ or }\langle t,t \rangle \modelsf \varphi_2\label{eq:lem:42}\\
\text{iff }&t \not\modelscl \varphi_1\text{ or }t \modelscl \varphi_2\label{eq:lem:43}\\
\text{iff }&t\modelscl \varphi_1 \rightarrow \varphi_2\label{eq:lem:44}
          \end{align}
          \begin{itemize}
           \item Equivalence between \eqref{eq:lem:41} and \eqref{eq:lem:42} holds by definition of the satisfaction relation
           \item Equivalence between \eqref{eq:lem:42} and \eqref{eq:lem:43} holds by induction hypothesis
           \item Equivalence between \eqref{eq:lem:43} and \eqref{eq:lem:44} holds by definition of the classical satisfaction relation
          \end{itemize}
          \item (Induction step Lemma~\ref{lem:htcc:modelscl}) For conditional constraint atom $c$,
          we get
          \begin{align}
             &\langle t,t \rangle \modelsf c\label{eq:lem:51}\\
  \text{iff }&t\in\den{\evalf{t}{t}(c[\cterm{r_1}{s_1}{\varphi_1},\dots,\cterm{r_n}{s_n}{\varphi_n}])}\label{eq:lem:52}\\
  \text{iff }&t\in\den{c[\evalf{t}{t}(\cterm{r_1}{s_1}{\varphi_1}),\dots,\evalf{t}{t}(\cterm{r_n}{s_n}{\varphi_n})]}\label{eq:lem:evaleqstep}\\
  \text{iff }&t\in\den{c[\evalcl{t}(\cterm{r_1}{s_1}{\varphi_1}),\dots,\evalcl{t}(\cterm{r_n}{s_n}{\varphi_n})]}\label{eq:lem:evalcleqstep}\\
  \text{iff }&t\in\den{\evalcl{t}(c[\cterm{r_1}{s_1}{\varphi_1},\dots,\cterm{r_n}{s_n}{\varphi_n}])}\label{eq:lem:53}\\
  \text{iff }&t\modelscl c \label{eq:lem:54}            
          \end{align}
          \begin{itemize}
           \item 
          Equivalence between \eqref{eq:lem:51} and \eqref{eq:lem:52} holds by definition of the satisfaction relation
           \item 
          Equivalence between \eqref{eq:lem:52} and \eqref{eq:lem:evaleqstep} holds by definition of the evaluation function
	   \item
          Equivalence between \eqref{eq:lem:evaleqstep} and \eqref{eq:lem:evalcleqstep} holds since 
          \begin{align*}
          &c[\evalf{t}{t}(\cterm{r_1}{s_1}{\varphi_1}),\dots,\evalf{t}{t}(\cterm{r_n}{s_n}{\varphi_n})]=\\
          &\quad c[\evalcl{t}(\cterm{r_1}{s_1}{\varphi_1}),\dots,\evalcl{t}(\cterm{r_n}{s_n}{\varphi_n})]) 
          \end{align*} by induction hypothesis that $\langle t,t \rangle\models\varphi_i$ iff $t\modelscl\varphi_i$ for $1\leq i\leq n$
           \item 
          Equivalence between \eqref{eq:lem:evalcleqstep} and \eqref{eq:lem:53} holds by definition of the evaluation function 
           \item 
          Equivalence between \eqref{eq:lem:53} and \eqref{eq:lem:54} holds by definition of the classical satisfaction relation
          \end{itemize}
      \end{itemize}
\end{itemize}

==> proofs/proof_prop_grounding_assigments.tex <==
\begin{proof}[Proof of Proposition~\ref{prop:grounding.assigments}]
First note that $d = \beta \models \df{\beta}$
and, thus, each implication of the form of~\eqref{eq:prop:grounding.assigments}
is equivalent to
\begin{gather}
\alpha = d \ \leftarrow \ d = \beta \wedge \varphi \wedge \df{\beta}
	\label{eq:prop:grounding.assigments.2}
\end{gather}
Let $\Gamma'$ be the set of all the implications of the form of~\eqref{eq:prop:grounding.assigments.2}
for all $d \in \D$.
Then, $\Gamma \equiv \Gamma'$ and we will show that $\Gamma' \equiv \gamma$.
Let $\tuple{h,t}$ be an interpretation.
Then, $\tuple{h,t} \models \gamma$ holds
iff one of the following conditions hold:
\begin{enumerate}
\item $\tuple{h,t} \models \alpha = \beta$
\label{eq:1:prop:grounding.assigments}
	\begin{itemize}
	\item This holds iff $h(\alpha) = h(\beta) \neq \undefined$
	\\iff there is some $d' \in \D$ such that 
	$h(\alpha) = h(\beta) = d'$
	\\iff there is some $d' \in \D$ s.t. $h(\alpha) = d'$
	and $h(\beta) = d'$
	\end{itemize}

\item $\tuple{t,t} \not\models \varphi \wedge \df{\beta}$
\label{eq:2:prop:grounding.assigments}
	\begin{itemize}
	\item This holds iff either $\tuple{t,t} \not\models \varphi$ or $t(\beta) = \undefined$
	\end{itemize}

\item both $\tuple{t,t} \models \alpha = \beta$ and $\tuple{h,t} \not\models \varphi \wedge \df{\beta}$
\label{eq:3:prop:grounding.assigments}
	\begin{itemize}
	\item This holds iff there is some $d' \in \D$ such that\\
	$t(\alpha) = d'$ and\\
	$t(\beta) = d'$ and\\
	either $\tuple{h,t} \not\models \varphi$ or $h(\beta) = \undefined$
	\end{itemize}
\end{enumerate}


Similarly, $\tuple{h,t} \models \Gamma$ iff for all $d \in \D$, one of the following conditions hold:
\begin{enumerate}[start=4]
\item $\tuple{h,t} \models \alpha = d$
	\label{eq:4:prop:grounding.assigments}
	\begin{itemize}
	\item This holds iff $h(\alpha) = d$
	\end{itemize}

\item $\tuple{t,t} \not\models d = \beta \wedge \varphi \wedge \df{\beta}$
	\label{eq:5:prop:grounding.assigments}
	\begin{itemize}
	\item This holds iff either $\tuple{t,t} \not\models \varphi$ or $t(\beta) \in \Du \setminus\{ d \}$
	\end{itemize}

\item both $\tuple{t,t} \models \alpha = \beta$ and 
$\tuple{h,t} \not\models d = \beta \wedge \varphi \wedge \df{\beta}$
	\label{eq:6:prop:grounding.assigments}
	\begin{itemize}
	\item This holds iff $t(\alpha) = d$ and\\
	either $h(\beta) \in \Du\setminus\{d\}$ or
	$\tuple{h,t} \not\models \varphi$
	\end{itemize}
\end{enumerate}
Hence, $\tuple{h,t} \models\gamma$ implies that Conditions~~\ref{eq:1:prop:grounding.assigments}-~\ref{eq:3:prop:grounding.assigments} hold.
Condition~\ref{eq:1:prop:grounding.assigments} implies 
Condition~\ref{eq:4:prop:grounding.assigments} for $d = d'$
and
Condition~\ref{eq:5:prop:grounding.assigments} for every~$d \in \D \setminus\{ d' \}$.
Furthermore,
Conditions~\ref{eq:2:prop:grounding.assigments} 
and Condition~\ref{eq:3:prop:grounding.assigments}
respectively imply Conditions~\ref{eq:4:prop:grounding.assigments} and~\ref{eq:6:prop:grounding.assigments}
for all $d \in \D$.
From this we get that
$\tuple{h,t} \models\gamma$
implies
$\tuple{h,t} \models\Gamma'$
and, thus, that $\gamma \models \Gamma$.
\\[5pt]
The other way around.
Assume $\tuple{h,t} \not\models \gamma$
and, thus, that Conditions~\ref{eq:1:prop:grounding.assigments}-\ref{eq:3:prop:grounding.assigments}
do not hold.
Then, the following conditions hold
\begin{enumerate}[ label=\arabic*'. , ref=\arabic*' ]
\item $h(\alpha) \neq d$ or $h(\beta) \neq d$ for every $d \in \D$
\label{eq:1':prop:grounding.assigments}

\item $\tuple{t,t} \models \varphi$ and $t(\beta) \neq \undefined$
\label{eq:2':prop:grounding.assigments}

\item either $t(\alpha) \neq d$ or $t(\beta) \neq d$  for every $d \in \D$, or\\
	both $\tuple{h,t} \models \varphi$ and $h(\beta) \neq \undefined$
\label{eq:3':prop:grounding.assigments}
\end{enumerate}
Let $d = t(\beta)$ and let us show that $\tuple{h,t}$ does not satisfy~\eqref{eq:prop:grounding.assigments.2}.
Note that we get $t(\beta) \in \D$ because of Condition~\ref{eq:2':prop:grounding.assigments}.
Furthermore, 
Condition~\ref{eq:2':prop:grounding.assigments}
also implies that $\tuple{t,t} \models \varphi$
and, thus, that Condition~\ref{eq:5:prop:grounding.assigments}
does not hold.
From Condition~\ref{eq:3':prop:grounding.assigments}
plus $d = t(\beta)$,
we get
\begin{enumerate}[ label=\arabic*''. , ref=\arabic*'' ]
\item either $t(\alpha) \neq d$ or
	both $\tuple{h,t} \models \varphi$ and $h(\beta) \neq \undefined$
\label{eq:3'':prop:grounding.assigments}
\end{enumerate}
The former, $t(\alpha) \neq d$, implies that Conditions~\ref{eq:4:prop:grounding.assigments} and~\ref{eq:6:prop:grounding.assigments} do not hold.
Furthermore, 
$\tuple{h,t} \models \varphi$ and $h(\beta) \neq \undefined$
imply that Condition~\eqref{eq:6:prop:grounding.assigments} does not hold.
Note that $t(\beta) = d$ and $h(\beta) \neq \undefined$
imply that $h(\beta) = d$.
Finally, from Condition~\ref{eq:1':prop:grounding.assigments}
plus $h(\beta) = d$ we get that $h(\alpha) \neq d$.
This implies that Condition~\eqref{eq:4:prop:grounding.assigments} does not hold.
Hence, $\tuple{h,t} \not\models \gamma$
implies that $\tuple{h,t} \not\models \Gamma'$
and we conclude that $\Gamma \equiv \gamma$.
\end{proof}

==> proofs/proof_prop_grounding_equality.tex <==
\begin{proof}[Proof of Proposition~\ref{prop:grounding.equality}]
First note that it is enough to show the result holds for the case in which the relation~$\prec$ is $\leq$ because the other cases are defined in terms of it.
Let $\tuple{h,t}$ be any interpretation such that
$h(x_i) \in \{ d_{i1}, \dotsc d_{in_i}, \undefined \}$
for every $x_i$.
Then,
$\tuple{h,t} \models c$
if and only if
$$
\tuple{h,t} \models \tau_{11} + \dotsc + \tau_{1n_1} + \dotsc + \tau_{m1} + \dotsc + \tau_{mn_m} \leq d_0
$$
with each $\tau_{ij} = \cterm{d_{ij}}{0}{x_i = d_{ij} \wedge \psi_i \wedge \df{d_{ij}}}$.
This holds
iff
\begin{gather}
\tuple{h,t} \models \tau'_{11} + \dotsc + \tau'_{1n_1} + \dotsc + \tau'_{m1} + \dotsc + \tau'_{mn_m} \leq d_0
	\label{eq:1:prop:grounding.equality}
\end{gather}
with each $\tau_{ij}' = \cterm{d_{ij}}{0}{x_i = d_{ij} \wedge \psi_i}$.
Note that $\df{d_{ij}} \equiv \top$ because $d_{ij}$ is a value.
Furthermore, \eqref{eq:1:prop:grounding.equality} holds
iff
\begin{gather*}
h(\eval{h}{t}{(\tau_{11}')}) + \dotsc + h(\eval{h}{t}{(\tau_{mn_m}')}) \leq d_0
\end{gather*}
iff
\begin{gather}
\eval{h}{t}{(\tau_{11}')} + \dotsc + \eval{h}{t}{(\tau_{mn_m}')} \leq d_0
	\label{eq:2:prop:grounding.equality}
\end{gather}
Note that $h(d_{ij}) = d_{ij}$ and $h(0) = 0$ because both are values.
\\[5pt]
On the other hand, $\tuple{h,t} \models c'$ iff
$$\tuple{h,t} \models \tau_1'' + \dotsc + \tau_m''\leq d_0$$
with each $\tau_i'' = \cterm{x_i}{0}{\psi_i \wedge \df{x_i}}$.
This holds iff
\begin{gather}
h(\eval{h}{t}{(\tau_1'')}) + \dotsc + h(\eval{h}{t}{(\tau_m'')}) \leq d_0
	\label{eq:3:prop:grounding.equality}
\end{gather}
Hence, we only need to show that~\eqref{eq:2:prop:grounding.equality} and~\eqref{eq:3:prop:grounding.equality} are equivalent
and, for this, it is enough to show, for every $i \in \{1, \dotsc, m \}$,
that
$$\eval{h}{t}{(\tau_{ij}')} = h(\eval{h}{t}{(\tau_i'')})$$
for some $j \in \{1,\dotsc,n_i \}$
and
$$\eval{h}{t}{(\tau_{ik}')} = 0$$
for every $k \neq j$.
By definition,
we get
\begin{align*}
\eval{h}{t}(\tau_{ij}')
&=
\left\{
\begin{array}{ll}
  d_i & \text{if } \langle h,t\rangle\models x_i = d_{ij} \wedge \psi_i\\
  0 & \text{if } \langle t,t\rangle\not\models x_i = d_{ij} \wedge \psi_i\\
  \undefined & \text{otherwise}
\end{array}
\right.
\end{align*}
and
\begin{align*}
h(\eval{h}{t}(\tau_i''))
&=
\left\{
\begin{array}{ll}
  h(x_i) & \text{if } \langle h,t\rangle\models \psi_i \wedge \df{x_i}\\
  0 & \text{if } \langle t,t\rangle\not\models \psi_i \wedge \df{x_i}\\
  \undefined & \text{otherwise}
\end{array}
\right.
\end{align*}
We now proceed by cases.
\begin{enumerate}
\item Assume that interpretation $\tuple{h,t}$ satisfies
$x_i = d_{ij} \wedge \psi_i$
for some value $d_{ij}\in \{ d_{i1}, \dotsc d_{in_i} \}$.
This implies $\tuple{h,t} \models  \psi_i \wedge \df{x_i}$
and, thus, we get
$$\eval{h}{t}(\tau_{ij}') = d_{ij} = h(x_i) = h(\eval{h}{t}(\tau_i''))$$
Furthermore, since $d_{ij} \neq d_{ik}$ for every $j \neq k$, this also implies that
$$\eval{h}{t}(\tau_{ik}') = 0$$
Hence, the result holds.

\item If $t(x_i) = \undefined$ or $\tuple{t,t} \not\models \psi_i$, then
we get that $\tuple{t,t}$ does not satisfy $x_i = d_{ij} \wedge \psi_i$
for every $d_{ij} \in \{ d_{i1}, \dotsc d_{in_i} \}$
and also that
$\tuple{t,t} \not\models \psi_i \wedge \df{x_i}$.
Therefore, it follows that
$$\eval{h}{t}(\tau_{ij}') = h(\eval{h}{t}(\tau_i'')) = 0$$
for every $j \in \{1, \dotsc, n_i \}$.

\item If we have
$t(x_i) = d_{ij}$ for some value $d_{ij}\in \{ d_{i1}, \dotsc d_{in_i} \}$
and
\mbox{$\tuple{t,t} \models \psi_i$}
and
$\tuple{h,t} \not\models \psi_i$,
then
\begin{align*}
\eval{h}{t}(\tau_{ij}') &= \undefined = h(\eval{h}{t}(\tau_i''))
\\
\eval{h}{t}(\tau_{ik}') &= 0
\end{align*}

\item Finally,
if we have
$t(x_i) = d_{ij}$ for some $d_{ij}\in \{ d_{i1}, \dotsc d_{in_i} \}$
and
$h(x_i) = \undefined$
and
$\tuple{h,t} \models \psi_i$,
then
\begin{align*}
\eval{h}{t}(\tau_{ij}') &= \undefined = h(\eval{h}{t}(\tau_i''))
\\
\eval{h}{t}(\tau_{ik}') &= 0
\end{align*}
\end{enumerate}
Therefore the result holds.
\end{proof}

==> proofs/proof_prop_htcc_reduct.tex <==
\begin{itemize}
  \item \textbf{Proof of Proposition~\ref{prop:htcc:reduct}}
    \begin{itemize}
        \item We proof Proposition~\ref{prop:htcc:reduct} via induction over the structure of the formula
        \item Lemma~\ref{lem:htcc:confree} constitutes the induction base of this proof
        \item (Induction step) For $\varphi=(\varphi_1 \otimes \varphi_2) \text{ and } \otimes \in \{\land,\lor,\rightarrow\}$, 
              we refer to the respective induction steps in the proof of Lemma~\ref{lem:htcc:confree}
              since the steps are independent of $\varphi_1$ and $\varphi_2$ being condition-free 
        \item (Induction step) For conditional constraint atom $c$,
          we get
      \begin{align}
                & \langle h,t\rangle\modelsf c \label{eq:prop:1} \\
\text{iff } & h\in\den{\evalf{h}{t}(c[\cterm{r_1}{s_1}{\varphi_1},\dots,\cterm{r_n}{s_n}{\varphi_n}])}\label{eq:prop:2}\\
&\text{ and } t\in\den{\evalf{t}{t}(c)}\nonumber  \\
\text{iff } & h\in\den{c[\evalf{h}{t}(\cterm{r_1}{s_1}{\varphi_1}),\dots,\evalf{h}{t}(\cterm{r_n}{s_n}{\varphi_n})]}\label{eq:propht}\\
&\text{ and } t\in\den{\evalf{t}{t}(c)}\nonumber \\
\text{iff } & h\in\den{c[\evalcl{h}(\cterm{r_1}{s_1}{\varphi_1^t}),\dots,\evalcl{h}(\cterm{r_n}{s_n}{\varphi_n^t})]}\label{eq:propfer}\\
&\text{ and } t\in\den{\evalcl{t}(c)} \nonumber\\
\text{iff } & h\in\den{\evalcl{h}(c[\cterm{r_1}{s_1}{\varphi_1}]\dots[\cterm{r_n}{s_n}{\varphi_n}]^t)}\label{eq:prop:3}\\
&\text{ and } t\in\den{\evalcl{t}(c)}  \nonumber\\
\text{iff } & h\modelscl c^t\text{ and }t\modelscl c  \label{eq:prop:4}\\
\text{iff } & h\modelscl c^t \label{eq:prop:5}
      \end{align}
      \begin{itemize}
           \item 
          Equivalence between \eqref{eq:prop:1} and \eqref{eq:prop:2} holds by definition of the satisfaction relation
           \item 
          Equivalence between \eqref{eq:prop:2} and \eqref{eq:propht} holds by definition of the evaluation function
	   \item 
	  The equivalence between \eqref{eq:propht} and \eqref{eq:propfer} holds, 
	  first, by induction hypothesis since  
	  \begin{align*}
	  &c[\evalf{h}{t}(\cterm{r_1}{s_1}{\varphi_1}),\dots,\evalf{h}{t}(\cterm{r_n}{s_n}{\varphi_n})]=\\
	  &\quad c[\evalcl{h}(\cterm{r_1}{s_1}{\varphi_1^t}),\dots,\evalcl{h}(\cterm{r_n}{s_n}{\varphi_n^t})]
	  \end{align*}
	  in case that $\langle h,t \rangle\modelsf\varphi_i$ iff $h\modelscl\varphi_i^t$ for $1\leq i \leq n$,
	  and second, since $\evalf{t}{t}(c)=\evalcl{t}(c)$ by Lemma~\ref{lem:htcc:evalcl}
           \item 
          Equivalence between \eqref{eq:propfer} and \eqref{eq:prop:3} holds by definition of the evaluation function
           \item 
          Equivalence between \eqref{eq:prop:3} and \eqref{eq:prop:4} holds by definition of the classical satisfaction relation
           \item 
          Equivalence between \eqref{eq:prop:4} and \eqref{eq:prop:5} holds by definitions of reduct and classical satisfaction relation
          since if $h\modelscl c^t$, $t\modelscl c$ has to hold as well because no valuation satisfies $\bot$
      
      \end{itemize}
    \end{itemize}
\end{itemize}

==> proofs/proof_thm_casp.tex <==

\begin{proof}[Proof of Theorem~\ref{thm:casp}]
Follows directly from Theorem~1 in~\cite{cakaossc16a}
and the fact that for condition-free free programs our semantics coincide with the one defined there.
\end{proof} 

